Efficiently-Verifiable Strong Uniquely Solvable Puzzles and Matrix Multiplication

We advance the Cohn-Umans framework for developing fast matrix multiplication algorithms. We introduce, analyze, and search for a new subclass of strong uniquely solvable puzzles (SUSP), which we call simplifiable SUSPs. We show that these puzzles are efficiently verifiable, which remains an open question for general SUSPs. We also show that individual simplifiable SUSPs can achieve the same strength of bounds on the matrix multiplication exponent $\omega$ that infinite families of SUSPs can. We report on the construction, by computer search, of larger SUSPs than previously known for small width. This, combined with our tighter analysis, strengthens the upper bound on the matrix multiplication exponent from $2.66$ to $2.505$ obtainable via this computational approach, and nears the results of the handcrafted constructions of Cohn et al.

==> implementation.tex <==
\subsection{Implementation}
\label{sec:implementation}

\subsubsection{Parallel matching implementation on Cuda}
	
	%https://ieeexplore.ieee.org/document/6012868

To make use of the available resources, we chose to implement a parallelized algorithm of \textproc{simplify} on the CUDA computing platform. Since CUDA operates on the SIMD paradigm (loosely speaking), parts of the algorithm would have to be vectorized in order to be effectively accelerated. At the high level, the procedure can be broken down into more easily parallelizable parts: initializing projection faces of the input graph $G$, decomposing each of the three faces into strongly connected components, calculating edges to remove in each projected graph, and finally updating $G$ with changes. The SCC decomposition algorithm can be redesigned as described in the paper [...]. Once the components are computed, edges of the 3D graph can be accordingly updated in parallel using every pair of vertices that are not in the same SCC. 

All of our algorithms are run experimentally on Ubuntu environment, Intel(R) Core(TM) i5-7500 CPU @ 3.40GHz processor with 16 GiB of RAM, and GeForce GTX 1060 6GB. We compared the performance of our parallel algorithm of \textproc{simplify} with the sequential implementation for puzzles up to size of 196. On average, the CUDA version was able to achieve a speed up by a factor of 10. The completely code and benchmarking utility will be made available on GitHub.
